Collapsing Molecular Clouds with Tracer Particles: Part I, What Collapses?

To understand the formation of stars from clouds of molecular gas, one essentially needs to know two things: What gas collapses, and how long it takes to do so. We address these questions by embedding pseudo-Lagrangian tracer particles in three simulations of self-gravitating turbulence. We identify prestellar cores at the end of the collapse, and use the tracer particles to rewind the simulations to identify the preimage gas for each core at the beginning of each simulation. This is the first of a series of papers, wherein we present the technique and examine the first question: What gas collapses? For the preimage gas at the t=0, we examine a number of quantities; the probability distribution function (PDF) for several quantities, the structure function for velocity, several length scales, the volume filling fraction, the overlap between different preimages, and fractal dimension of the preimage gas. Analytic descriptions are found for the PDFs of density and velocity for the preimage gas. We find that the preimage of a core is large and sparse, and we show that gas for one core comes from many turbulent density fluctuations and a few velocity fluctuations. We find that binary systems have preimages that overlap in a fractal manner. Finally, we use the density distribution to derive a novel prediction of the star formation rate.

==> Report.tex <==
Dear Dr Collins,

Copied below are the comments on your manuscript entitled "Collapsing Molecular Clouds with Tracer Particles: Part I, What Collapses?", ref. MN-22-3569-MJ, which you submitted to Monthly Notices of the Royal Astronomical Society.

Minor revision of your manuscript is requested before it is accepted for publication. Providing these changes are made, we should be able to send your revised version directly to our publisher without further review.

You should submit your revised version, together with your response to any comments from the editor and reviewer at https://urldefense.com/v3/__https://mc.manuscriptcentral.com/mnras__;!!PhOWcWs!0h7yd_nqy97rkAm-ubscxk38edRKFHp9wxM8TNPCbB3OAEOEbwvApjJBkLq7fgNp8bGI1mYYACiZaaHQjjJuR_VZoXja$  . The deadline for this is six months from today.

Enter your Author Centre, where you will find your manuscript title listed under "Manuscripts with Decisions". Under "Actions," click on "Create a Revision". Please ensure that you also respond to any comments from the editor or assistant editor.

IMPORTANT: do not submit your revised manuscript as a new paper!

When submitting your revised manuscript, you should only upload clean files (remove any bold font/track changes) for our publishers, as accepted manuscripts are now immediately published online ahead of the proof-corrected version.

We look forward to receiving your revised manuscript.

Regards,

Claire Williams (in Anna's absence)

Anna Evripidou (Ms)
Senior Assistant Editor
Monthly Notices
Royal Astronomical Society
Email: aevripidou@ras.ac.uk
Tel: +44 (0)1483 536 737

This message is confidential and is intended solely for the use of the individual(s) to whom it is addressed.  If you have received this message in error, do not open any attachment but please notify the sender (above) and delete this message from your system.

cc: all listed co-authors




Assistant Editor's Comments:

Please use keywords from the MNRAS keywords list only on your manuscript. Please see https://urldefense.com/v3/__https://academic.oup.com/mnras/pages/general_instructions*6.1__;Iw!!PhOWcWs!0h7yd_nqy97rkAm-ubscxk38edRKFHp9wxM8TNPCbB3OAEOEbwvApjJBkLq7fgNp8bGI1mYYACiZaaHQjjJuRy34XKl2$   Layout for more information on keywords. 

Please ensure that all textual labels in figures are at least as large as the caption text; any smaller and they become too difficult to read. 


Scientific Editor's (Andrew King) Comments:

(There are no comments.)


Reviewer's Comments:

This is an interesting paper and a novel idea to trace back gas elements that end
up in star-forming cores. I recommend publishing nearly as is. I have a few small
concerns that may be just typos.

Equation (4) has a separation D, which, if the units are distance, makes the
equation incorrect. What is D? Is the particle separation D*Delta x? Is D a
relative parameter?

For equation 22, is the velocity dispersion supposed to vary as the square root of
the length, in which case p=1?

The main result is that the key indicator for future presence in a star-forming
core is high density, but perhaps this is because the simulation is limited in
time and that time corresponds to a lower density limit. The authors state that
later times would have the un-collapsed gas disbursed by feedback, which is
reasonable, but this dispersal is not guaranteed as the inward flow could occupy a
small angular scale with high ram pressure and the outward flow a large angular
scale with low ram pressure (as in the spoke and hub model). If accretion to cores
continues longer, would this density predictor still be valid?

I note a similar use of density as a probability for the appearance of young stars
in Elmegreen (2018 ApJ 854:16; section 5.2).

==> Response.tex <==
Dear Anonymous Referee--

Thank you for your response to our paper.  We shall address your questions.

Q1 "Equation (4) has a separation D, which, if the units are distance, makes the
equation incorrect. What is D? Is the particle separation D*Delta x? Is D a
relative parameter?"

That is correct, it makes more sense if we say "a separation D $\Delta x$".  We have made this change.

Q2: "For equation 22, is the velocity dispersion supposed to vary as the square root of
the length, in which case p=1?"

You are correct, we have fixed the 0.5.

Q4: The main result is that the key indicator for future presence in a star-forming
core is high density, but perhaps this is because the simulation is limited in
time and that time corresponds to a lower density limit. The authors state that
later times would have the un-collapsed gas disbursed by feedback, which is
reasonable, but this dispersal is not guaranteed as the inward flow could occupy a
small angular scale with high ram pressure and the outward flow a large angular
scale with low ram pressure (as in the spoke and hub model). If accretion to cores
continues longer, would this density predictor still be valid?

This is a very interesting question.  To really answer it we'll need to do more simulations, which we'll do in a future work.   I suspect that further accretion would come mostly from gas that's close to the core, which mostly comes from the same convex hull that we have found. In this case, more accretion would simply be sampling the PDF of the convex hull better, and the result won't change.  

Though of course, $V(*|\rho)$ could get more shallow, as lower density gas falls on.  We do see ample evidence of small angle, high ram pressure gas that you mention (see Paper II!) so if there is more gas that will accrete that way, the result will change.  I suspect that all the gas that can cause spoke-and-hub style accretion has already landed on the dense spots by this time, but that's speculative.


Q5: I note a similar use of density as a probability for the appearance of young stars
in Elmegreen (2018 ApJ 854:16; section 5.2).

That is a useful reference, we have added a citation.

==> mnras_toc.tex <==

% The MNRAS class isn't designed to include a table of contents, but for this document one is useful.
% I therefore have to do some kludging to make it work without masses of blank space.
\begingroup
\let\clearpage\relax
\tableofcontents
\endgroup
\newpage

